Proof Hints for Event-B

Interactive proofs are often considered as costs of formal modelling activity. In an incremental development environment such as the Rodin platform for Event-B, information from proof attempts is important input for adapting the model. This paper considers the idea of using interactive proofs to "improve" the model, in particular, to convert them into automatic ones. We propose to lift some essential proof information from the interactive proofs into the model as what we called proof hints. In particular, proof hints are not only for the purpose of proofs: it helps to understand the formal models better.

==> Makefile <==
##### User customisation
# The main LaTeX file
main_latex_name ?= proof-hints

# The BiBTeX file
bib_name ?= proof-hints

# LaTeX program
latex_program ?= $(PDFLATEX)
#####

# All the *.tex files
all_files.tex ?= $(wildcard *.tex)

default: $(main_latex_name).pdf

$(main_latex_name).pdf: $(main_latex_name).bbl $(all_files.tex)
	$(QUIET)\
	$(call show-info, $(main_latex_name)".tex --> "$(main_latex_name)".pdf");\
	$(call run-latex-silence, $(main_latex_name));\
	if ! $(EGREP) -q 'LaTeX Error:' $(main_latex_name).log; then \
		if $(EGREP) -q 'LaTeX Warning: There were undefined references.' $(main_latex_name).log; then \
			$(call show-info, $(bib_name)".bib --> "$(main_latex_name)".bbl");\
			$(call run-bibtex, $(main_latex_name));\
			$(call show-info, $(main_latex_name)".tex --> "$(main_latex_name)".pdf");\
			$(call run-latex-silence, $(main_latex_name));\
		fi;\
		if $(EGREP) -q 'Rerun to get cross-references right.' $(main_latex_name).log; then \
			$(call show-info, $(main_latex_name)".tex --> "$(main_latex_name)".pdf");\
			$(call run-latex, $(main_latex_name));\
		fi;\
	fi

$(main_latex_name).bbl: $(bib_name).bib
	$(QUIET)\
	$(call show-info, $(main_latex_name)".tex --> "$(main_latex_name)".pdf");\
	$(call run-latex-silence, $(main_latex_name));\
	$(call show-info, $(bib_name)".bib --> "$(main_latex_name)".bbl");\
	$(call run-bibtex, $(main_latex_name))


.PHONY: clean cleanall

clean:
	$(QUIET)\
	rm -f *.aux *.blg *.log *.nav *.out *.rel *.snm *.toc *.synctex.gz

cleanall: clean
	$(QUIET)\
	rm -f $(main_latex_name).bbl;\
	rm -f $(main_latex_name).pdf


# Programs
SED		?= sed
BIBTEX	        ?= bibtex
PDFLATEX        ?= pdflatex -file-line-error -halt-on-error
EGREP           ?= egrep
# == Makefile Color Output ==
TPUT		?= tput

#
# User-settable definitions
#
LATEX_COLOR_WARNING	?= magenta
LATEX_COLOR_ERROR	?= red
LATEX_COLOR_INFO	?= green
LATEX_COLOR_UNDERFULL	?= blue
LATEX_COLOR_OVERFULL	?= red bold
LATEX_COLOR_SUCCESS	?= green bold
LATEX_COLOR_FAILURE	?= red bold

# $(call get-term-code,codeinfo)
# e.g.,
# $(call get-term-code,setaf 0)
get-term-code = $(shell $(TPUT) $1)

black	:= $(call get-term-code,setaf 0)
red	:= $(call get-term-code,setaf 1)
green	:= $(call get-term-code,setaf 2)
yellow	:= $(call get-term-code,setaf 3)
blue	:= $(call get-term-code,setaf 4)
magenta	:= $(call get-term-code,setaf 5)
cyan	:= $(call get-term-code,setaf 6)
white	:= $(call get-term-code,setaf 7)
bold	:= $(call get-term-code,bold)
uline	:= $(call get-term-code,smul)
reset	:= $(call get-term-code,sgr0)


# Gets the real color from a simple textual definition like those above
# $(call get-color,ALL_CAPS_COLOR_NAME)
# e.g., $(call get-color,WARNING)
get-color	= $(subst $(space),,$(foreach c,$(LATEX_COLOR_$1),$($c)))

C_WARNING	:= $(call get-color,WARNING)
C_ERROR		:= $(call get-color,ERROR)
C_RESET		:= $(reset)
C_INFO          := $(call get-color,INFO)
C_UNDERFULL     := $(call get-color,UNDERFULL)
C_OVERFULL      := $(call get-color,OVERFULL)

# Colorize BiBTeX output.
color_bibtex := \
$(SED) \
-n \
-e '/Warning--.*/ s/.*/$(C_WARNING)&$(C_RESET)/ p' \
-e '/.*---.*/,/.*skipping whatever remains of this entry/ s/.*/$(C_ERROR)&$(C_RESET)/ p'

# Colorize LaTeX output.
color_latex := \
$(SED) \
-n \
-e '/.*Warning:.*/,/^$$/ s/.*/$(C_WARNING)&$(C_RESET)/ p' \
-e '/.*Error:.*/,/^$$/ s/.*/$(C_ERROR)&$(C_RESET)/ p' \
-e '/Underfull.*/,/^$$/ s/.*/$(C_UNDERFULL)&$(C_RESET)/ p' \
-e '/Overfull.*/,/^$$/ s/.*/$(C_OVERFULL)&$(C_RESET)/ p'

color_latex_error := \
$(SED) \
-n \
-e '/.*Error:.*/,/^$$/ s/.*/$(C_ERROR)&$(C_RESET)/ p'

# BibTeX invocations
#
# $(call run-bibtex,<tex stem>)
run-bibtex = $(BIBTEX) $1 | $(color_bibtex)

# PDFLaTeX invocations
#
# $(call run-pdflatex,<tex stem>)
run-latex = $(latex_program) $1 | $(color_latex)

# PDFLaTeX invocations silence
#
# $(call run-pdflatex-silence,<tex stem>)
run-latex-silence = $(latex_program) $1 | $(color_latex_error)

# Show info message
#
# $(call show-info,<text message>)
show-info = echo $1 | $(SED) -e 's/.*/$(C_INFO)&$(C_RESET)/'

QUIET	:= @
